UrBench: A Comprehensive Benchmark for Evaluating Large Multimodal Models in Multi-View Urban Scenarios

Recent evaluations of Large Multimodal Models (LMMs) have explored their capabilities in various domains, with only few benchmarks specifically focusing on urban environments. Moreover, existing urban benchmarks have been limited to evaluating LMMs with basic region-level urban tasks under singular views, leading to incomplete evaluations of LMMs' abilities in urban environments. To address these issues, we present UrBench, a comprehensive benchmark designed for evaluating LMMs in complex multi-view urban scenarios. UrBench contains 11.6K meticulously curated questions at both region-level and role-level that cover 4 task dimensions: Geo-Localization, Scene Reasoning, Scene Understanding, and Object Understanding, totaling 14 task types. In constructing UrBench, we utilize data from existing datasets and additionally collect data from 11 cities, creating new annotations using a cross-view detection-matching method. With these images and annotations, we then integrate LMM-based, rule-based, and human-based methods to construct large-scale high-quality questions. Our evaluations on 21 LMMs show that current LMMs struggle in the urban environments in several aspects. Even the best performing GPT-4o lags behind humans in most tasks, ranging from simple tasks such as counting to complex tasks such as orientation, localization and object attribute recognition, with an average performance gap of 17.4%. Our benchmark also reveals that LMMs exhibit inconsistent behaviors with different urban views, especially with respect to understanding cross-view relations.

==> figures/dataset_comparison.tex <==


\begin{table}[h]
  \centering
  \caption{The comparison of benchmarks for remote sensing related evaluation, general evaluation, and urban related evaluation.}
  % \resizebox{0.45\textwidth}{!}{
  \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{llllll}
    % {lp{1.2cm}lp{1.2cm}lp{1.8cm}l}
    % {llllll}
    \hline
    Dataset   & Size        & View          & Image          & Source           & Answer        \\
    \hline
    RSVQA     & $>$ 1M      & Satellite           & Single         & OSM              & Open          \\
    EarthVQA  & $>$ 100K    & Satellite           & Single         & Repurposed              & Open          \\
    VRSBench  & $>$ 100k    & Satellite           & Single         & Annotated              & \makecell[l]{Open, \\BBox, \\Caption} \\  MUIRBench & 2.6K        & Street           & Interleave          & Text             & Multi-choice            \\
    MMBench   & 3K          & -             & Single         & Repurposed              & Multi-choice            \\
    MMMU      & 11.5K       & -             & Interleave          & Annotated              & Open          \\
    \hline
    CMBench & 13.4K       & \makecell[l]{Street, \\ Satellite}      & Interleave           & \makecell[l]{OSM, \\Repurposed, \\Annotated}      & \makecell[l]{Open, \\ Multi-choice}   \\
    \hline
    \end{tabular}
  }

  \label{tab:dataset_comparison}
\end{table}

==> figures/dataset_statistics.tex <==
% \begin{table}[htbp]
%   \centering
%   \caption{The detailed statistics of CityBench from question and image level. Note that }
  % \resizebox{0.9\textwidth}{!}{
  \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{llcc}
    %表格第一条线和最后一条要加粗，中间的两根也加粗换成一根
    \toprule
    \multicolumn{2}{c}{Question}                          & Test      & Val \\
    \hline
    \multicolumn{2}{c}{Total}                                   & 10483     & 1117 \\
    \hline
    % \multirow{5}[0]{*}{view type}       & cross-view            & 4522      & 488 \\
    %                                     & satellite-view        & 3181      & 354 \\
    %                                     & mono-street-view      & 3259      & 325 \\
    %                                     % street-view 要拆分开
    %                                     & panoramic-street-view & 2131      & 253 \\
    %                                     & multi-street-view     & 231       & 21 \\
    \multirow{5}[0]{*}{View Type}       & cross            & 4208      & 434 \\
                                        & sat        & 2618      & 268 \\
                                        & mono-str      & 1694      & 195\\
                                        % street-view 要拆分开
                                        & pano-str & 1735      & 196 \\
                                        & multi-str     & 228       & 24 \\                                        
                                        
    \hline
    % \multirow{2}[0]{*}{visual prompt}   & with visual prompt    & 5667      & 621 \\
    %                                     & without visual prompt & 7657      & 820 \\
    \multirow{2}[0]{*}{Visual Prompt}   & with    & 4227      & 446 \\
                                        & without & 6256      & 671 \\                                        
    \hline
    \multirow{2}[0]{*}{Answer Type}     & MC       & 8920      & 964 \\
                                        & open            & 1563      & 153 \\
                                        % & caption               & 1178      & 109 \\
    \hline
    \multirow{4}[0]{*}{Images per Q}    & 1 image               & 5522      & 606 \\
                                        & 2 images              & 3485      & 357 \\
                                        & 4 images              & 753       & 77 \\
                                        & 5 images              & 723       & 77 \\
    % \toprule
    % \multicolumn{2}{c}{Image Level}                             & test      & val \\
    % \hline
    % \multicolumn{2}{c}{total}                                   & 8142      & 1320 \\
    % \hline
    % \multirow{3}[0]{*}{view type}       & mono-street-view      & 1574      & 277 \\
    %                                     & panoramic-street-view & 3026      & 483 \\
    %                                     & satellite-view        & 3542      & 560 \\
    % \hline
    % \multirow{2}[0]{*}{visual prompt}   & with visual prompt    & 2568      & 463 \\
    %                                     & with and without prompt & 4628    & 818 \\
    %                                     & without visual prompt & 946       & 39 \\
    % \hline
    % \multirow{5}[0]{*}{source}          & in-house              & 6085      & 941 \\
    %                                     & Vigor                 & 483       & 102  \\
    %                                     & Cityscapes            & 494       & 168  \\
    %                                     & Mapillary Traffic Sign& 447       & 53 \\
    %                                     & IM2GPS                & 633       & 56 \\
    %                                     % & Img2GPS\_SAT          & 618?      & 68? \\
    %                                     % % % 下边这行合并到前两行去
    %                                     % & Ig2GPS\_SAT,Img2GPS   & 627       & 59 \\
    \bottomrule
    \end{tabular}%
    }
%   \label{tab:statistics}%
% \end{table}%


==> figures/evalTableWithViews.tex <==
\begin{table*}[htbp]
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccc|c|c|c|c|cc|ccc}
    \toprule
    \multirow{3}[6]{*}{Model} & \multicolumn{6}{c|}{Geo-Localization}          & \multicolumn{6}{c}{Object Understanding} \\
\cmidrule{2-13}          & \multicolumn{3}{c|}{CR} & IR    & CL    & OR    & OM    & \multicolumn{2}{c|}{OG} & \multicolumn{3}{c}{OAR} \\
\cmidrule{2-13}          & satellite & street  & cross & cross & cross & cross & cross & satellite & street & satellite & street & cross \\
    \midrule
    GPT-4o & \textbf{66.1}  & \textbf{84.8}  & \textbf{86.4}  & \textbf{85.9}  & \underline{35.3}  & \underline{30.7}  & 28.0  & \underline{62.3}  & 36.0  & 43.8  & 58.9  & \textbf{48.8}  \\
    Gemini-1.5-Flash & 59.3  & 71.6  & 77.8  & 25.9  & 25.9  & 24.0  & 22.0  & 55.9  & 27.9  & 36.2  & 51.5  & 37.9  \\
    Claude-3.5-Sonnet & 59.2  & \underline{74.2}  & \underline{83.3}  & 55.8  & 30.8  & \textbf{33.3}  & 22.0  & \textbf{81.5}  & \textbf{48.0}  & \textbf{50.9}  & 43.2  & \underline{43.7}  \\
    \midrule
    TinyLLaVA & 48.9  & 53.8  & 53.0  & 23.2  & 24.7  & 27.9  & 22.9  & 54.6  & 32.0  & 26.5  & 31.9  & 7.8  \\
    InternVL2-2B & 40.3  & 56.4  & 53.9  & 23.8  & 31.9  & 29.0  & 25.5  & 29.1  & 31.1  & 39.6  & 50.5  & 35.6  \\
    InternVL2-4B & 43.9  & 62.5  & 58.3  & 24.2  & 27.4  & 23.1  & 30.6  & 34.4  & 27.3  & 33.3  & 50.9  & 38.2  \\
    XComposer-4KHD & 53.6  & 66.2  & 65.7  & 26.0  & 27.5  & 25.9  & 16.2  & 53.5  & 35.2  & 45.2  & \textbf{64.9}  & 38.3  \\
    LLaVA-NeXT-7B-Mistral & 45.7  & 52.5  & 56.5  & 25.9  & 24.2  & 24.0  & \textbf{43.9}  & 36.6  & 30.8  & 26.3  & 31.9  & 31.0  \\
    LLaVA-NeXT-7B-Vicuna & 46.1  & 51.1  & 56.5  & 24.6  & 27.2  & 23.3  & 31.8  & 28.9  & 26.1  & 23.1  & 28.9  & 38.3  \\
    InstructBLIP-Vicuna-7B & 35.1  & 44.1  & 41.9  & 25.7  & 25.4  & 27.1  & 22.9  & 25.3  & 20.9  & 19.6  & 21.3  & 14.0  \\
    LLaVA-NeXT-8B & 48.5  & 54.4  & 60.2  & 27.0  & 27.8  & 26.0  & \underline{39.8}  & 44.7  & 39.7  & 23.1  & 26.1  & 32.5  \\
    InternVL2-8B & 37.2  & 61.6  & 53.5  & 26.6  & 31.8  & 25.2  & 30.3  & 32.2  & 31.8  & 34.2  & 49.3  & 40.9  \\
    Idefics-2-8B & 57.9  & 67.5  & 70.9  & 23.8  & 26.0  & 24.1  & 24.8  & 15.4  & 24.9  & 23.6  & 37.2  & 24.3  \\
    LLaVA-NeXT-13B & 42.6  & 54.1  & 59.1  & 24.5  & 27.7  & 26.7  & 31.8  & 48.0  & 25.9  & 24.3  & 29.6  & 25.7  \\
    InternVL2-26B & 53.1  & 66.4  & 64.4  & 23.0  & 32.3  & 24.7  & 26.1  & 39.2  & 36.0  & 43.4  & \underline{64.5}  & 42.7  \\
    LLaVA-NeXT-34B & 47.9  & 65.1  & 62.1  & 26.0  & 28.5  & 27.8  & 28.7  & 47.3  & 36.0  & 24.7  & 33.0  & 19.0  \\
    LLaVA-NeXT-Interleave-7B & 54.4  & 58.3  & 60.8  & 41.6  & 27.6  & 25.5  & 37.3  & 38.8  & 36.7  & \underline{45.6}  & 47.9  & 35.9  \\
    Mantis-LLaMA3-SigLIP & 63.3  & 67.4  & 70.3  & 32.4  & 27.0  & 27.2  & 25.2  & 44.0  & 27.6  & 40.0  & 37.4  & 38.6  \\
    Mantis-Idefics2 & \underline{64.4}  & 70.3  & 72.1  & 29.9  & 27.0  & 25.7  & 29.6  & 52.7  & 27.8  & 34.6  & 41.7  & 32.8  \\
    VILA-1.5-13B & 53.9  & 65.8  & 68.2  & 33.7  & 28.6  & 24.1  & 25.8  & 29.3  & 34.2  & 38.2  & 47.2  & 33.3  \\
    VILA-1.5-40B & 60.7  &\underline{74.2}  & 75.4  & \underline{62.5}  & \textbf{36.8}  & 27.9  & 34.1  & 59.7  & \underline{40.6}  & 39.3  & 50.7  & 33.6  \\
    \bottomrule
    \end{tabular}
    }
  % \caption{The LMMs experimental results of the different views of tasks under Geo-Localization and Object Understanding evaluation dimensions. The maximum value and the next largest value of each task are indicated by the \textbf{bold} and \underlined{underlined} text, respectively. Task names are abbreviated for brevity.}
  \caption{The LMMs experimental results of the different views of tasks under Geo-Localization and Object Understanding evaluation dimensions. The maximum value and the next largest value of each task are indicated by the \textbf{bold} and \underline{underlined} text, respectively. Task names are abbreviated for brevity.}
  \label{tab:app_result_gl_ou}
\end{table*}

\begin{table*}[htbp]
  \centering
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|ccc|cc|c|cc}
    \toprule
    \multirow{3}[5]{*}{Model} & \multicolumn{3}{c|}{Scene Reasoning} & \multicolumn{8}{c}{Scene Understanding} \\
\cmidrule{2-12}          & RBR   & TSR   & VPR   & \multicolumn{3}{c|}{SR} & \multicolumn{2}{c|}{RU} & CO    & \multicolumn{2}{c}{SC} \\
\cmidrule{2-12}          & street & street & street & satellite & street & cross & satellite & street & satellite & satellite & street \\
    \midrule
    GPT-4o & \textbf{79.6}  & \underline{68.2}  & \textbf{77.9}  & 61.7  & \textbf{61.3}  & \textbf{71.9}  & 42.4  & \underline{86.4}  & 40.1  & \underline{79.2}  & \textbf{78.6}  \\
    Gemini-1.5-Flash & 77.8  & \textbf{75.8}  & 69.8  & 59.6  & 54.7  & 59.5  & 40.5  & \textbf{87.4}  & 29.1  & 68.3  & 65.5  \\
    Claude-3.5-Sonnet & 73.7  & 37.7  & 66.7  & \underline{64.7}  & 52.6  & 40.0  & \textbf{54.7}  & 67.7  & \textbf{48.0}  & \textbf{84.0}  & 70.0  \\
    \midrule
    TinyLLaVA & 40.3  & 32.7  & 48.6  & 17.5  & 7.2   & 1.1   & 3.9   & 47.4  & 9.5  & 27.4  & 28.6  \\
    InternVL2-2B & 64.8  & 45.9  & 54.5  & 47.5  & 45.9  & 50.3  & 20.2  & 52.6  & 28.6  & 30.8  & 27.7  \\
    InternVL2-4B & 73.0  & 56.6  & 62.6  & 51.9  & 51.9  & 53.0  & 36.6  & 52.6  & 22.1  & 36.1  & 51.8  \\
    XComposer-4KHD & 75.5  & 62.6  & 60.8  & 54.1  & 52.5  & 60.0  & \underline{49.0}  & 53.5  & 35.8  & 26.4  & 44.6  \\
    LLaVA-NeXT-7B-Mistral & 59.2  & 42.7  & 45.5  & 55.2  & 50.8  & 60.5  & 38.8  & 52.6  & 34.1  & 28.6  & 27.7  \\
    LLaVA-NeXT-7B-Vicuna & 49.6  & 51.5  & 54.5  & 56.3  & 51.4  & 60.5  & 28.5  & 52.6  & 34.3  & 25.2  & 28.6  \\
    InstructBLIP-Vicuna-7B & 30.7  & 25.7  & 29.3  & 36.1  & 35.9  & 27.0  & 14.4  & 0.0   & 20.4  & 27.6  & 29.5  \\
    LLaVA-NeXT-8B & 55.2  & 52.8  & 58.6  & 60.1  & 48.6  & 58.4  & 40.6  & 52.6  & 37.3  & 23.0  & 27.7  \\
    InternVL2-8B & 74.9  & 54.8  & 62.6  & 54.6  & 50.3  & 54.1  & 37.6  & 70.6  & 27.4  & 49.6  & 58.0  \\
    Idefics2-8B & 64.7  & 60.4  & 42.8  & 50.8  & 51.4  & 54.6  & 34.6  & 52.6  & 22.9  & 28.8  & 24.1  \\
    LLaVA-NeXT-13B & 54.0  & 52.1  & 52.3  & 54.6  & 52.5  & 54.6  & 41.5  & 52.6  & 34.1  & 23.5  & 31.3  \\
    InternVL2-26B & \underline{77.9}  & 63.8  & \underline{71.2}  & \textbf{68.3}  & \underline{58.0}  & \underline{68.6}  & 32.1  & 53.1  & \underline{43.0}  & 49.4  & 64.3  \\
    LLaVA-NeXT-34B & 65.6  & 59.3  & 56.8  & 58.5  & 54.1  & 62.2  & 41.1  & 52.6  & 25.9  & 49.6  & 69.6  \\
    LLaVA-NeXT-Interleave-7B & 65.8  & 55.9  & 63.1  & 55.2  & 45.9  & 56.8  & 38.9  & 33.8  & 27.4  & 46.2  & 56.3  \\
    Mantis-LLaMA3-SigLIP & 67.6  & 41.6  & 57.7  & 62.8  & 51.9  & 62.7  & 32.4  & 23.9  & 28.2  & 49.6  & 62.5  \\
    Mantis-Idefics2 & 68.9  & 50.6  & 56.3  & 53.0  & 48.6  & 49.2  & 33.6  & 59.6  & 30.1  & 52.8  & 67.9  \\
    VILA-1.5-13B & 66.3  & 43.8  & 46.4  & 50.3  & 43.6  & 49.2  & 31.0  & 54.8  & 21.6  & 46.7  & 55.4  \\
    VILA-1.5-40B & 76.4  & 55.5  & 61.3  & 59.0  & 48.1  & 53.5  & 35.6  & 70.2  & 32.1  & 64.6  & \underline{74.1}  \\
    \bottomrule
    \end{tabular}
    }
  \caption{The LMMs experimental results of the different views of tasks under Scene Reasoning and Scene Understanding evaluation dimensions. The maximum value and the next largest value of each task are
indicated by the \textbf{bold} and \underline{underlined} text, respectively. Task names are abbreviated for brevity.}
  \label{tab:app_result_sr_su}
\end{table*}

